CoMet: Modeling Group Cohesion for Socially Compliant Robot Navigation in Crowded Scenes

We present CoMet, a novel approach for computing a group's cohesion and using that to improve a robot's navigation in crowded scenes. Our approach uses a novel cohesion-metric that builds on prior work in social psychology. We compute this metric by utilizing various visual features of pedestrians from an RGB-D camera on-board a robot. Specifically, we detect characteristics corresponding to proximity between people, their relative walking speeds, the group size, and interactions between group members. We use our cohesion-metric to design and improve a navigation scheme that accounts for different levels of group cohesion while a robot moves through a crowd. We evaluate the precision and recall of our cohesion-metric based on perceptual evaluations. We highlight the performance of our social navigation algorithm on a Turtlebot robot and demonstrate its benefits in terms of multiple metrics: freezing rate (57% decrease), deviation (35.7% decrease), and path length of the trajectory(23.2% decrease).

==> old_Background.tex <==
\section{Background}
In this section, we justify our choice of macroscopic and microscopic features used in our work using the research in psychology. We then define the symbols and notations used in our formulation, and formally explain our person detection and tracking process. 

\subsection{Selected Features for Cohesion Estimation}
We choose to use multiple features for perceived group cohesion estimation due to their benefits and success in affective computing applications such as emotion recognition \cite{emoticon}. In addition, using multiple features is beneficial when the detectability of these features varies continuously in dynamic settings. 

\subsubsection{Proximity Between Group Members} \label{sec:hall's-proxemics}
Proximity is chosen based on the proxemics principles established by Edward T. Hall \cite{hall-proxemics}. His theory states that humans have three distinct spaces while interacting with others: 1. intimate space ($<$ 45cms from a person), 2. social and consultative space (120-200cms), and 3. public space ($>$200cms). We generalize this idea to unstructured social scenarios where people walk, stand or sit together. People maintain a lower proximity from people with whom they have a close relationship ($\implies$ high cohesion).

% While the threshold distance for each space could vary slightly based on cultural expectations, this idea of social distance is observed universally.


\subsubsection{Walking Speed, Group Size, and Gender} \label{sec:speed-dyads-gender}
\cite{friendly-dyads} studied individual and mixed gender groups' walking speeds in a controlled environment and observed significantly slower speeds when people walk with their romantic partners. \cite{group-permeability} analyzed the perceptions of people when passing through a group of two and four people in a university hallway. It was observed people tended to penetrate through the 4-person group fewer times than over a 2-person group. We draw the following assertions from the above research: 1. a slower-than-average walking speed in a group (specifically in mixed-gender groups) indicates a close relationship between group members (high cohesion), and 2. humans perceive the cohesion of a bigger group to be higher (lower permeability) than a smaller group. Based on these inferences, we choose to detect walking speeds, group size, and gender to better estimate group cohesion.

% In \cite{walking-behavior-ped-groups}, it is observed that dyads and triads of friends tend to walk side by side, whereas larger friend groups walk in V-formations that facilitate better interactions between group members. 
% \cite{interpersonal-distance-group-walking} analyzed 1,020 groups and concluded that mixed-gender dyads of friends walked alongside each other more often than same-gender dyads. 

\subsubsection{Interactions Based on Face Pose} \label{sec:interaction}
In this work, we specifically focus on jointly-focused interactions \cite{interaction-1961} because these entail a sense of mutual activity and engagement between people and imply their willingness to focus their attention on others. We extrapolate this to signify a higher level of cohesion between them. Visually, interactions can be detected by estimating peoples' 3-D face poses \cite{interaction-murino,head-pose} and detecting when the vectors point towards each other. 

\subsection{Symbols, Definitions and Assumptions}
A list of symbols frequently used in this work is shown in Table \ref{tab:symbol_defn}. We define a few symbols where they are used for better readability. We use the terms person and pedestrian interchangeably, and \textit{i}, \textit{j}, and \textit{k} to represent indices. All distances, angles and velocities are measured relative to a rigid coordinate frame attached to the camera (on the robot) capturing the scene. The X-axis of this frame points outward from the camera and the Y-axis points to the right, with its origin at the center of the image. We also assume that a continuous stream of RGB and depth images with the same dimensions for a given scene are available. The time interval between two consecutive RGB images in the stream is $\Delta t$. 

\begin{table}[]
\centering
\begin{tabularx}{\linewidth}{|c|L|} % Change the alignment to center
\hline
\textbf{Symbols} & \textbf{Definitions}  \\
\hline
$[x^{i, t}, y^{i, t}]$ & Position vector of person i at time t relative to the camera coordinate frame. \\
\hline
$\textbf{v}^{i, t}$ & Walking velocity vector of person i at time t relative to the camera coordinate frame. $\textbf{v}^{i, t} = [\Dot{x}^{i, t}, \Dot{y}^{i, t}]$ \\
\hline
$I_{rgb}^t$ & RGB image captured at time instant t of width w and height h. \\
\hline
$I_{depth}^t$ & Depth image captured at time instant t of width w and height h. \\
\hline
% $\Delta t$ & Time interval between two subsequent RGB frames. \\ 
% \hline
$\bb{B}^i$ & Bounding box of person with ID i. \\
\hline
$[x^{\bb{B}^i}_{cen}, y^{\bb{B}^i}_{cen}]$ & Centroid of the bounding box $\bb{B}^i$. \\
\hline
$\mathbf{x}^{i, t}$ & State vector used in Kalman filter for walking vector estimation for person i at time instant t. $\mathbf{x}^{i, t} = [x^{i, t} \,\, y^{i, t} \,\, \Dot{x}^{i, t} \,\, \Dot{y}^{i, t}]^T$ \\
\hline
$ID^t$ & Set of person IDs detected in $I^t_{rgb}$. \\
\hline
$n^k$ & Number of members in Group $G^{k,t}$. \\
\hline
N & Number of people detected in an RGB image. \\
\hline
$\mathbf{f}_o^i$ & Unit vector of person i's face relative to the camera coordinate frame. \\ 
% $\textbf{f}^i = [f_x^i \, f_y^i \, f_z^i]^T$. \\
\hline
\begin{tabular}{@{}c@{}}$K_p, K_w, K_s$ \\ $K_i, K_g$ \end{tabular} & Weighing constants for each feature \\
\hline
% $comfort(i, j)$ & Function that measures the level of comfort between persons i and j. \\
% \hline
% $detectability of $
\end{tabularx}
\caption{\small{List of symbols used in our work and their definitions.}}
\label{tab:symbol_defn}
\vspace{-15pt}
\end{table}

\subsection{Preliminaries for Person Localization} \label{sec:ped-localization}
The fundamental step in estimating group cohesion is to first detect, track and localize people relative to the camera frame in a continuous stream of RGB images. We use YOLOv5 \cite{yolo} and Deep Sort \cite{deepsort} to detect and track people respectively. YOLOv5 outputs a set of bounding boxes $\mc{B}= \{ \bb{B}^{i}$\} for each detected person i in an RGB image at time instant t ($I_{rgb}^t$). $\bb{B}^{i}$ is denoted using its top left and bottom right corners in pixel coordinated. In addition, it also assigns a unique integer number as an ID for each detected person. 

% , as $\mc{B}= \{ \bb{B}^{i} \ | \ \bb{B} = [x_{tl}, y_{tl}, x_{br}, y_{br}]\}$. Here $[x_{tl}, y_{tl}]$ denotes the top left corner, and $[x_{br}, y_{br}]$ denotes bottom right corner's pixel coordinates of the $i^{th}$ bounding box $\bb{B}^i$. 

Next, to accurately localize people, the distance of each detected person relative to the camera coordinate frame must be estimated at each time instant t. To this end, we use $I_{depth}^t$, whose every pixel contains the proximity (in meters) of an object at that location of the image. The pixels in $I_{depth}^t$ contain values between a minimum and maximum distance range, which depends on the camera used to capture the image.

% which are represented as,

% \vspace{-15pt}
% \begin{equation}
% \begin{split}
%     I_{depth}^t &= \{C \in \mathbb{R}^{w \times h} : offset < C_{ij} < range\}, \\
%     1 &\le i \le w \qquad \text{and} \qquad 1 \le j \le h,  
% \end{split}
%     \label{eqn:cam}
% \end{equation}

% \no where \textit{offset} is the minimum distance from the camera from which an object's proximity can be measured, and \textit{range} is the maximum distance the camera can measure in meters. In other words, each pixel in $I_{depth}^t$ contains the proximity (in meters) of an object at that location of the image.




==> old_Our_Method.tex <==
\section{Our Method: CoMet}


\subsection{Detecting Macroscopic Features}
To detect proximity, walking speed, dyads and triads, we need to estimate the distance between a pair of people, and the associated walking vectors. 

\subsubsection{Estimating Distance between People} 
To estimate the proximity between people at time instant t, first the detection bounding boxes from the RGB image passed through YOLOv5 are superimposed over the depth image. To estimate the distance of a person i ($d^{i, t}$) from the camera, the mean of all the pixel values within a small square centered around $[x^{\bb{B}^i, t}_{cen}, y^{\bb{B}^i, t}_{cen}]$ is computed.  The angular displacement $\psi^{i, t}$ of person i relative to the camera can be computed as, $\psi^{i, t} = \left(\frac{\frac{w}{2} - x^{\bb{B}^i, t}_{cen}}{w}\right) * FOV_{RGBD}$. Here $FOV_{RGBD}$ is the field of view angle of the RGB-D camera. Person i's location relative to the camera can be computed as $[x^{i, t} \,\, y^{i, t}]$ = $d^{i, t}$ * [$\cos{\psi^{i, t}} \,\, \sin{\psi^{i, t}}$]. The distance between a pair of people i and j can then be computed as, $dist(i, j) = \sqrt{(x^{i, t} - x^{j, t})^2 + (y^{i, t} - y^{j, t})^2}$.

\vspace{10pt}

\subsubsection{Estimating Walking Vectors} \label{sec:walk-vec} 
To estimate the vector $\mathbf{v}^i$ which represents person i's walking trajectory in $I^t_{rgb}$, we use a Kalman filter with a constant velocity motion model. All the detected people in $I^t_{rgb}$ (with their IDs stored in the set $ID^t$) are modeled using the state vector $\mathbf{x}^t$ defined in Table \ref{tab:symbol_defn}. If $ID^t$ contains IDs which were not present in $ID^{t - \Delta t}$, we initialize their corresponding state vectors $\mathbf{x}^t$ with constant values. For all the people who were detected in previous RGB images, i.e., with previously initialized states, we update their states using the standard Kalman prediction and update the steps \cite{kalman-filter}. We use a zero mean Gaussian noise with a pre-set variance to model the process and sensing noise.  

% The final step in the state estimation is,
% \vspace{-10pt}
% \begin{equation}
%     \mathbf{x}^{i, t} =  \mathbf{x}^{i, t - \Delta t} + K^{i, t}   \qquad \forall i \in ID^{t - \Delta t} \cap ID^{\Delta t}.  
% \end{equation}


\subsubsection{Group Detection}
Let us consider any set of people's IDs $G^{k, t} \subseteq ID^t$. At any time t, if the following conditions hold,
\vspace{-10pt}

\begin{equation}
    \begin{split}
        dist(i, j) \le \Gamma \quad \forall \, i, j \in G^{k, t} \\
        \sign\left(\frac{\textbf{v}^i \cdot \textbf{v}^j}{\|\textbf{v}^i\| \|\textbf{v}^j\|}\right) > 0 \quad \forall \, i, j \in G^{k, t},
    \end{split}
\end{equation}

\no then the set $G^{k, t}$ is classified as a \textit{group} in the image $I^t_{rgb}$. Here, $\Gamma$ is a distance threshold set manually and $\sign()$ is the signum function. The first condition ensures that people are close to each other, and the second condition ensures that the group members walk in the same direction. 

\subsection{Macroscopic Components of Cohesion}
We now discuss how the detected macroscopic features can be used for cohesion estimation.

\subsubsection{Proximity Cohesion Score} 
We use the average distance between group members to model the Hall's proxemics theory as previously extrapolated. As observed in Section \ref{sec:hall's-proxemics}, cohesion between people is inversely proportional to the distance between them. Therefore, the cohesion score due to proximity is formulated as,

\vspace{-10pt}
\begin{equation}
C_p(G^{k, t}) = K_p \cdot \frac{n^k}{\sum\limits_{\substack{i, j \in G^{k, t} \\ i \ne j}} dist(i, j)}. 
% detectability(proximity) \propto \frac{1}{d^i_{cam} + d^j_{cam}}.
\label{eqn:prox-cohesion}
\end{equation}

The RHS of Equation \ref{eqn:prox-cohesion} is the reciprocal of the average distance between members in group $G^{k, t}$. 

\subsubsection{Walking Speed Cohesion Score} 
Based on the discussion in Section \ref{sec:speed-dyads-gender}, we next compare the average walking speeds of each group with the average walking speed of all the detected people in $I^t_{rgb}$. Therefore, the cohesion score for a walking group ($\|\textbf{v}^j\| \ne 0 \,\, \forall j \in G^{k, t}$) due to its walking speed is formulated as,

\vspace{-10pt}
\begin{equation}
% \begin{split}
    C_w(G^{k, t}) = K_w \cdot \left( \frac{\sum\limits_{\forall i \in ID^t} \|\textbf{v}^i\|}{N} \right) / \left( \frac{\sum\limits_{\forall j \in G^{k, t}} \|\textbf{v}^j\|}{n^k} \right) \\
    % \sum\limits_{\forall j \in G^{k, t}}\|\textbf{v}^j\| \ne 0.
% \end{split}
\label{eqn:walk-speed-cohesion}
\end{equation}

\no This reflects assertion 2 made in Section \ref{sec:speed-dyads-gender}, since cohesion is inversely proportional to walking speed. The average walking speed of the entire scene is included in this formulation to normalize out the effects of crowding in the scene. If $\sum\limits_{\forall j \in G^{k, t}}\|\textbf{v}^j\| = 0$, i.e., the group is static, then $C_w(G^{k, t}) = K_w \cdot \eta$, where $\eta$ is a user-set large constant value. 

\subsubsection{Group Size Cohesion Score}
Based on assertion 1 in Section \ref{sec:speed-dyads-gender}, the certainty of the computed cohesion for a group is inversely dependent on the group size. Therefore, we compute the cohesion score for a group due to its size as,

\begin{equation}
    C_s(G^{k, t}) = K_s \cdot n^k.
    \label{eqn:grp-size-cohesion}
\end{equation}

% Group size is used as an assistive feature to indicate the level of confidence in the comfort score computed using the other macroscopic features. 

%%%%%%%%%%%%%%%%%%%%%%% MICROSCOPIC FEATURES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Detecting Microscopic Features}
In this section, we explain how interactions using face poses and genders of group members are detected.  

\subsubsection{Detecting Interactions}
We use two 3-D vectors to represent the position and orientation of a person's face. We use OpenFace \cite{openface} to localize person i's face position relative to the camera coordinate frame ($\mathbf{f}_p^i$) and to obtain a unit vector ($\mathbf{f}_o^i$) for the face orientation. Two individuals are considered to be interacting if their face positions and orientations satisfy the following condition:

\begin{equation}
    \|\mathbf{f}_p^i - \mathbf{f}_p^j \|_2 > \|\mathbf{f}_p^i + \mathbf{f}_o^i - (\mathbf{f}_p^j + \mathbf{f}_o^j) \|_2 .
    \label{eqn:interaction-condition}
\end{equation}

\no This condition checks whether two people's heads are facing each other, with the reasonable assumption that non-interacting people typically do not face each other.  

\subsubsection{Detecting Gender}
Several methods exist which use a person's face to predict their gender. However, in many scenarios, the person's face could be too small and not visible. Therefore, we use the approach detailed in \cite{SMPL-X:2019}, a pre-trained ResNet18 gender classifier which takes a person's full-body color image, and OpenPose \cite{openpose} joints as inputs and labels the gender of the detected person. 

\subsection{Microscopic Components of Cohesion}
We now discuss the contributions of these microscopic features in the overall cohesion model. 

\subsubsection{Interaction Cohesion Score}
% Intuitively, and as explained in Section \ref{sec:interaction}, the level of comfort between two or more people depends on the duration of interaction between them. 
The interaction condition between any two people in a group (equation \ref{eqn:interaction-condition}) can be applied to all pairs in a group and it's contribution to the cohesion score of a group can be written as:

\begin{equation}
    C_i(G^{k, t}) =  K_i \cdot \frac{1}{n^k} \cdot \sum\limits_{\substack{i \ne j \\ i, j \in G^{k, t} }}\frac{\sign(\theta_{ij})}{\cos{\theta_{ij}}}.
    \label{eqn:interaction-cohesion}
\end{equation}

% This corresponds to the reciprocal of the average value of $\cos{\theta}$ between all the pairs of people in a group. Where $\theta$ is the angle between the face vectors of a pair of people. 
\no Here $\theta_{ij}$ is the angle between vectors $\mathbf{f}_o^i$ and $\mathbf{f}_o^j$.
Since $\frac{\cos{\theta}}{\sign(\theta)} \in (-1, -\frac{1}{\sqrt{2}}] \cup [\frac{1}{\sqrt{2}}, 1]$ when $\theta \in [-\frac{\pi}{4}, \frac{\pi}{4}]$ $\implies \frac{\sign(\theta)}{\cos{\theta}} \in [-\sqrt{2}, -1) \cup [1, \sqrt{2}]$. Intuitively, the cohesion score is positive, when people are facing towards each other, and negative otherwise. 

\vspace{5pt}
\subsubsection{Gender Cohesion Score}
We quantify gender as a two-valued variable and use it as an assistive feature to walking speed and group size in the overall cohesion score. That is, 

\vspace{-10pt}
\begin{equation}
    C_g(G^{k, t}) =  
    \begin{cases}
        1 \quad \text{if} \,\, G^{k, t} \text{ members are of same gender}, \\
        K_g \quad \text{if} \,\, G^{k, t} \text{ is a mixed-gender group.}
    \end{cases}
    \label{eqn:gender-cohesion}
\end{equation}

This is based on assertion 1 in \ref{sec:speed-dyads-gender}. Its overall contribution can be seen in equation \ref{eqn:final-score}.

\subsection{CoMet and Relationship Classification}
% Add details about the detectability of a feature. 
% Talk about limiting the value of each term between a range.
% Talk about the 3 categories. 
% Talk about setting thresholds for 3 categories.
Using the individual cohesion scores in equations \ref{eqn:prox-cohesion}, \ref{eqn:walk-speed-cohesion}, \ref{eqn:grp-size-cohesion},\ref{eqn:interaction-cohesion},\ref{eqn:gender-cohesion}, the total cohesion score for a group at time t ($G^{k, t}$) is given as,

\begin{equation}
% \begin{split}
    C_{tot}(G^{k, t}) = (C_p + C_g \cdot (C_w + C_s) + C_i)/d^{k,t}_min.
% \end{split}
\label{eqn:final-score}
\end{equation}

\no Here, $G^{k, t}$ is omitted in the RHS for readability. If any of these features is not detectable, their contribution to the 


 
